Multi-view Kernel Completion

In this paper, we introduce the first method that (1) can complete kernel matrices with completely missing rows and columns as opposed to individual missing kernel values, (2) does not require any of the kernels to be complete a priori, and (3) can tackle non-linear kernels. These aspects are necessary in practical applications such as integrating legacy data sets, learning under sensor failures and learning when measurements are costly for some of the views. The proposed approach predicts missing rows by modelling both within-view and between-view relationships among kernel values. We show, both on simulated data and real world data, that the proposed method outperforms existing techniques in the restricted settings where they are available, and extends applicability to new settings.

==> exp.tex <==



\section{Numerical Experiments}

In this section we do comparative study of performance of the proposed method  with existing method which can perform the same task. 

 
\paragraph{Comparative Methods:}
\begin{itemize}
\item KNN(k) : This is a simplest k-nearest neighbour imputation of kernel rows/ columns.  For a missing data point $t$ in the $m^{th}$ view the k-nearest neighbour is selected according to kernel values of available views. Finally equal(KNN(k)) / wighted(WKNN(k)) importance weight of $\bA^{(m)}$ are assigned only for selected neighbours.
\item EM: Em based method to predict missing values in one kernel when one auxiliary view is present.
\item MKLpsd : Equation (\ref{eqn:pk2})
\item Nys-diff: Equation (\ref{eqn:pk5}) when different columns have been selected for different views
\item Nys-same:     Equation (\ref{eqn:pk5}) when same columns have been selected for different views
\item MKLapprox :  Equation (\ref{eqn:pk4})
\item Final : Equation (\ref{eqn:impute})
\end{itemize}
 
\paragraph{Dataset:}
\begin{itemize}
\item TOY data set :  all toy data sets contain 5 views data where 5 data point have no missing views and other 45 data points have missing views. The underlying sub-spases are aligned for view 1,3 and 2,4,5.  The kernel functions are following 
\begin{itemize}
\item TYOL:  Linear kernel for all views 
\item TOYGn: Gaussian kernel with width $n$ for all views
\item TOYLGn: Linear kernel for view 1,2 and 3  and Gaussian kernel for views 4 and 5
\end{itemize}  
\item DRMsmall : DREAM challenge 7 data with 8 original views 
\item Full Cream Challange data set with derived complex views by combining more than one of these original views
\item RCV : multi lingual data
\end{itemize}

\paragraph{Stability Checking for A}

It is not clear to me how to do this stability check up.

I did following experiments

I prepare data set as follows

\begin{itemize}
\item 3 data 2-d data points has been randomly generates (as shown in black in Figure (\ref{fig:A})
\item Randomly create 2 sets of 13 (3+10) datas points using two different embeddings based on these 3 data points. The embeddings are shown in 2nd rows of Figure \ref{fig:A}. 
\item 4 views are generated as following via linear transformation from 2-dim data from each embedding to 2-dim and 100-dim respectively. View 1 and 3 are from one embedding  and view 2 and 4 are from other. While view 1 and 2 have 2-dim feature-maps and view 3 and 4 have 100-dim. The distribution of kernel values is shown in Figure \ref{fig:Ak} 
\item I have also added 100 extra noisy dimension to view 3 and 4 and kernel values their are shown if Figure \ref{fig:Ak2}
\item Figure \ref{fig:Data1A} shows the relation between prediction loss of kernel values and prediction loss of across view relationship for both Equation(\ref{eon:impute}) and Equation(\ref{eqn:pk3})
\item Figure \ref{fig:Data1A} shows the relation between prediction loss of kernel values and prediction loss of across view relationship for both Equation(\ref{eon:impute}) and Equation(\ref{eqn:pk3}) for Noisy data set.
\item Observation: 
\begin{itemize}
\item Figure \ref{fig:Data1A} shows that approximation in kernel values is more for Equation(\ref{eqn:pk3}) than Equation(\ref{eon:impute})  after a proper running of parameters.
  Hence it is not a good idea to restrict  kernel values on convex hull  of other kernel values . While restricting each embedding in convex hull of  embedding of other views are helping in better approximation of kernel values.
\end{itemize}
\end{itemize}

\begin{figure}
\includegraphics[width = .45\textwidth]{data2v2.png}
\caption{Two different data sets(top row) have been generated using two different embeddings embeddings (bottom row)}
\label{fig:A}
\end{figure}

\begin{figure}
\includegraphics[width = .45\textwidth]{kernels.png}
\caption{Distribution of kernel values}
\label{fig:Ak}
\end{figure}

\begin{figure}
\includegraphics[width = .45\textwidth]{kernels2.png}
\caption{Distribution of kernel values}
\label{fig:Ak2}
\end{figure}

\begin{figure}
\includegraphics[width = .45\textwidth]{KvsS.png}
\includegraphics[width = .45\textwidth]{KvsA.png}
\includegraphics[width = .45\textwidth]{SvsA.png}
\caption{Relation between different losses for noisy data set}
\label{fig:Data2A}
\end{figure}
\begin{figure}
\includegraphics[width = .45\textwidth]{KvsS_noisy.png}
\includegraphics[width = .45\textwidth]{KvsA_noisy.png}
\includegraphics[width = .45\textwidth]{SvsA_noisy.png}
\caption{Relation between different losses}
\label{fig:Data1A}
\end{figure}

%\paragraph{Result/Observation}


\begin{center}
\includegraphics[width = .45\textwidth]{R.png}\\
\end{center}
\begin{center}
\begin{figure*}
\includegraphics[width = .8\textwidth]{sameK.png}\\
\end{figure*}
\begin{figure*}
\includegraphics[width = .8\textwidth]{diffK.png}\\
\end{figure*}
\begin{figure*}\includegraphics[width = .8\textwidth]{alldrmsmall.png}\\
\end{figure*}
\end{center}
\newpage

























==> exp_rmse_14jan.tex <==
\subsection{Comparison of  ability  to predict the missing kernels}
In this section we study the performance of all above mentioned methods in terms of ability  to predict the missing kernel rows on 7 synthetic and two real world data-sets. 
   \subsubsection{Average Relative Error}
   We evaluate the performances of all methods using the { \it average relative error} (ARE) by following \citet{xu13}. Let $\hat{\bK}^{(m)}_{t:}$ is the predicted $t^{th}$ row for $m^{th}$ view and corresponding true values of kernel row is ${\bK}^{(m)}_{t:}$ then we define the {\it relative error} as relative root mean square deviation  $\frac{\|\hat{\bK}^{(m)}_{t:}-{\bK}^{(m)}_{t:}\|_2}{\|{\bK}^{(m)}_{t:}\|_2}$ and finally we report the average over all missing data-points for a view.
   \begin{equation}
       \textrm{Average Relative Error (ARE) } = \frac{\sum_{t \notin I^{(m)}}\frac{\|\hat{\bK}^{(m)}_{t:}-{\bK}^{(m)}_{t:}\|_2}{\|{\bK}^{(m)}_{t:}\|_2}}{Nt^{(m)}}
       \label{eqn:are}
   \end{equation}
   Where $Nt^{(m)}$ is the number of unavailable data-points in the $m^{th}$ views.
   
   \subsubsection{Observation}
   \begin{figure*}
       \centering
       \includegraphics[width=1\textwidth]{TOYrmse3.png}
       \caption{Average relative error (Equation(\ref{eqn:are})) for all synthetic and DRM data set. All values are average over all views and also 10 random validation and test partition with 10 different missing entries}
       \label{fig:rmse}
   \end{figure*}
   
   Figure \ref{fig:rmse} shows performance of various \mkc\ methods varies with variation of eigen spectrum of kernel matrices across different views. All proposed \mkc\ methods predict missing values more accurately than Knn imputation and \emb\ for all kind of eigen spectrums and all amount of missing views. \emb has very high error and also high variance. \emht outperforms all other variants of \mkc\ in almost all the data-sets, while \psd\ outperform all other approximated methods when kernel functions are highly non-linear (TOYG0.1). We also observe that with increase of non-linearity in kernel values performance of all \mkc\ with approximation deteriorate. As underlying subspaces for all these toy data-sets are not same, hence \emhm\ always perform worse than \emht. Also advantage of \emht over \mkckernel\ can be observed for TOYLG1 data-sets when number of missing views are more ,i.e., 2 and 3. For this data-set different views have different kernel functions. \mkckernel\ restrict kernels of one view in convex hull of other relevant views, hence they are not able to model underlying subspace similarity and group the views according to kernel functions. To predict missing values of one Gaussian kernel (view 4 or view 5) it exploits available information in other views with same kernel function.% hence when both of these views are not available then they are not able to predict them accurately.
   On the other hand \emht\ are able to model similarity in underlying subspace structure and hence outperforms \mkckernel\ . 
   
   
   For DRM data-sets also \mkc s\ perform better than \emb\ and Knn methods. Considering performance over all views (Figure \ref{fig:rmse}) \emht\ performs best but \rnd\ is very close to it. As kernel function varies a lot for different views \mkckernel\ can not predict the missing kernel rows accurately specially for (see Figure \ref{fig:drm8data}) {\it exome sequence} and {\it binarized RNA sequencing data} views. Figure{fig:S} shows the predicting relevant views for \mkckernel\ and \emht\ for these two views.  This shows necessity of \emht\ for better modelling real world data-sets. While looking at view wise performance in Figure \ref{fig:DRM8}, we observe \mkc\ fails to predict kernel values of almost diagonal kernels on binarized exome sequence kernel (Figure \ref{fig:drm8data}) 
   
   \begin{figure*}
       \centering
       \includegraphics[width=1\textwidth]{DRM8rmse.png}
       \caption{View wise average relative error (Equation (\ref{eqn:are})) for DRM data-set. All values are average over all 10 random validation and test partition with 10 different missing entries.}
       \label{fig:DRM8}
   \end{figure*}
   \begin{figure}
       \centering
       \includegraphics[width=0.45\textwidth]{S.png}
       \caption{Figure showing pictorial representation of relevant view information predicted by \mkckernel\ and \emht\ }
       \label{fig:S}
   \end{figure}
   
   \subsection{Run time comparison of various \mkc method}
   Figure \ref{fig:time} shows advantage of with kernel approximation the kernel completion model \mkc \  is many times faster than the \psd\ . This gap increases with increase number of missing views.
   
   \begin{figure}
       \centering
       \includegraphics[width=0.45\textwidth]{runtime.png}
       \caption{Runtime of \mkc \ and \emb\ for all data-sets in second}
       \label{fig:time}
   \end{figure}

==> intro_old.tex <==
\section{Introduction}

\paragraph{Area:} In recent years, a great many methods have been proposed for multi-view learning , i.e,  learning from data collected from multiple sources  to utilize  the complimentary information generated from different sources \citet{sun13} where sources are also called as views. In the field of machine learning, data-points are utilized often to compute the similarity among them with some defined similarity measure and finally this similarity measures are enough for learning.  The kernelized method capture this similarity among data points in  kernel gram matrix and  the multiple kernel learning(MKL) framework  \citet{gon11} is popular way to accumulate  information from multiple sources where kernel gram matrices built on features from each individual views are combined for better learning.  MKL needs to know  full kernel matrices for individual view.  In case of multi-view learning , i.e.,  the learning with data from multiple sources, it is very natural that information from some sources are not available for some data points.  Incomplete-data problem exists in a wide range of fields, including social sciences, computer vision, biological systems, and remote sensing. For example some sensor can goes off for some random samples or the structural property of a protein with know sequence and functions may not be known yet. This introduces missing entries in view level, i.e, all features corresponding to a view for a data point can be  missing simultaneously.   Neglecting views with missing entries restricts models to exploit useful information collected from that view through the data points for which feature values corresponding to that view are known. 

\paragraph{Problem Definition}
In this paper, we propose a method to complete kernel matrices for individual views in multi-view data-set with missing values.  
The proposed method impute whole rows and columns of individual kernel matrices by utilizing information available from other views even if all available views have some missing entries in it.   

 \paragraph{Novelty in problem :}  \citet{tsu03} has proposed an EM based method to complete a kernel matrix corresponding to a view with missing entries with help of available a full kernel matrix from another auxiliary view. The problem we are solving here  differ from the problem they have solved in two ways : (1) Instead of completing kernel for individual view independently we collaboratively complete more than one incomplete kernel matrices corresponding to different  views with missing entries by sharing information among them.  (2) The proposed method does not require any complete kernel matrix.

\paragraph{Challenges:} Due to absence  of full rows/columns in incomplete kernel matrices, no existing single view kernel completion method can be applied to complete  kernel matrices of individual views independently.  Again, due to use of full Eigensystem of auxiliary full kernel matrix, \citet{tsu03} also can not be used to complete a kernel matrix with missing rows/columns when no other auxiliary complete kernel matrix is available.  On the other hand, generative models based method like \citet{lia15} is unable to model highly non-linear kernels like RBF as it assumes approximate kernel matrix for each view as linear kernel in some low dimensional space.

It is hard to propagate information across views in terms of Eigen system of kernel matrix when no kernel matrix is complete.  The main challenge for this project is to propagate necessary information form  incomplete kernel matrices  of other views to complete missing rows/columns of one kernel with high accuracy.
 
\paragraph{Technical contribution:} In this paper, we have proposed a novel method along with an efficient algorithm to complete all incomplete kernel matrices collaboratively through effective information propagation across views. Figure \ref{fig:model} shows a pictorial presentation of problem definition and our approach to solve it.  We exploit the concept of restricting completed kernel matrix of one view on convex hull of kernels of other related views following the multiple kernel learning method \citet{lan04,bac04}. Finally we extend this idea by restricting embeddings of one view on convex hull of embeddings of other views and learn completed kernel by learning underlying embedding of all views collectively. 

%We proposed the concept of using kernel subspace alignment for mutli-view  kernel completion task. 

Our approach of multi-view kernel completion through propagating relevant information across views, restrict the completed kernel matrix in a subspace of positive semidefinite cone. We restrict the individual normalized kernel matrix corresponding to each view on a convex hull of normalized kernel matrices of other views by following \citet{arg06} %which has used this kind of restriction for learning kernel from a set of kernel matrices. 



Restricting the  kernel of each view on the  convex hull of kernels of other views  restrict the kernel values  to have same underlying distribution for all views. It is useful to exploit across-view similarity among their underlying embeddings.  When modelling multi-view embedding \citet{she13} has assumed to have same local linear embedding in all views. But this restrict all embeddings are to be exactly same. To make our model enough flexible to capture the relationship of not only exactly same embeddings but also similar embeddings, we propose a novel approach of restricting  the embedding of one view on the convex hull of embeddings of other similar views.

It is important to note that the effective dimension of the intra - view embedded subspace depends on the number of feature-maps defining it and that varies across views depending on non-linearity of the corresponding kernel. The proposed model automatically decides upon the dimension of this subspace of individual views  while embedding all feature-maps into them and along with restricting it to be on the convex hull of embedding of homogeneous views. The non-linearity of individual kernel functions are also preserved in the kernel among bases which define the corresponding subspace.

Once we know the embeddings of data-points in an individual subspace of a view and the relationship among embeddings across the  homogeneous views,  we can extrapolate the position of one data-point in one view to another subspace of another view where its feature-map is missing. In this way we are able to embed all missing feature-maps in all views simultaneously even if  any complete kernel matrix is not available. 


As a result, the proposed model is not only able to model the highly non-linear kernels for individual views, it is also able to model non-linear relationships among kernels of different views.  Moreover, simultaneous prediction approach enable us to capture the required information from other views with missing values and it has no need of any complete view.  More importantly the predicted complete kernel gram matrix will also satisfy positive semi definite property without any explicit low rank assumption.

As the proposed model simultaneously learn  the view specific subspaces, embeddings of all data points on it by restricting it to be on convex hull of other related views,  solving this problem efficiently is a daunting task. We have defined a non-convex optimization problem but without  any positive semidefinite cone constraint which has been efficiently solved by  solving a sequence of convex problem.



==> intro_oldv2.tex <==
\section{Introduction}

In recent years, many methods have been proposed for multi-view learning, i.e,  learning with data collected from multiple sources or \enquote{views} to utilize  the complementary information in them. Kernelized methods capture the similarities among data points in a kernel matrix. The multiple kernel learning (MKL) framework  \citep{gon11} is a popular way to accumulate information from multiple sources, where kernel matrices built on features from individual views are combined for better learning.  MKL needs to know  full kernel matrices for each view.  In case of multi-view learning, it is common that information from some sources are not available for some data points.  

{\bf Motivation:} The incomplete-data problem exists in a wide range of fields, including social sciences, computer vision, biological systems, and remote sensing. Some sensors can go off for some random samples. When legacy data sets are integrated, some views may not have been measured for some data points. For instance, gene expression may have been measured for some of the examples, but not for others, and as biological sample has been exhausted, the missing measurements can't be made any more. On the other hand, some measurements may be too expensive to repeat for all samples;  e.g., patient's genotype may be measured only if a particular condition holds. All these examples introduce missing views, i.e, all features of a view for a data point can be  missing simultaneously. A few kernel completion approaches have been proposed  \citep{gra02,tsu03,lia15} (refs here), but none of the existing methods is applicable for our problem. 

%Neglecting views with missing entries restricts models to exploit useful information collected from that view through the data points for which feature values corresponding to that view are known.  

{\bf Novelty in problem definition:} In this paper, we propose a method to complete kernel matrices for individual views in multi-view data sets with missing values. The new method can process completely missing rows/columns in a kernel matrix. It does not require any of the kernel to be complete in contrast to some existing ones and is applicable to even highly non-linear kernels. These aspects make the proposed method attractive for practical applications. 

%\paragraph{Existing related methods:} \cite{gra02} proposed a semi-definite programming based method to complete individual kernel matrix when missing elements are few and distributed randomly. \citet{tsu03} has proposed an expectation maximization based method to complete a kernel matrix for a view with missing entry with the help of available a full kernel matrix from another auxiliary view.  On the other hand, \citet{lia15} proposed generative models based method to model similarity matrix approximating similarity matrix for each view as linear kernel in some low dimensional space. 

 
 
 %\citet{tsu03} has proposed an EM based method to complete a kernel matrix corresponding to a view with missing entries with help of available a full kernel matrix from another auxiliary view. The problem we are solving here  differ from the problem they have solved in two ways : (1) Instead of completing kernel for individual view independently we collaboratively complete more than one incomplete kernel matrices corresponding to different  views with missing entries by sharing information among them.  (2) The proposed method does not require any complete kernel matrix.

{\bf Challenges:} Due to absence  of full rows/columns in the incomplete kernel matrices, no existing single-view kernel completion method \citep{gra02,pai10} can be applied to complete  kernel matrices of individual views independently. In the multi view setting, \citet{tsu03} have proposed an expectation maximization based method to complete an incomplete kernel matrix for a view with the help of a complete kernel matrix from another view.  Due to use of full eigensystem of the auxiliary full kernel matrix, that method can't be used to complete a kernel matrix with missing rows/columns when no other auxiliary complete kernel matrix is available.  On the other hand, \citet{lia15} proposed generative model based method which approximates the similarity matrix for each view as a linear kernel in some low dimensional space. Therefore, it is unable to model highly non-linear kernels like RBF. % as it assumes approximate kernel matrix for each view as linear kernel in some low dimensional space. 

It is hard to propagate information across views in terms of the eigensystem of a kernel matrix when no kernel matrix is complete.  The main challenge in our problem is to propagate, with high accuracy, the information necessary to complete missing rows/columns of a kernel, from incomplete kernel matrices  of other views  .
 
{\bf Technical contribution:} In this paper, we propose a novel method to complete all incomplete kernel matrices collaboratively, by learning boht between-view and within-view relationship among the kernel values (Figure \ref{fig:model}).
%through effective information propagation across views along with learning within view relationship among kernel values (Figure \ref{fig:model}). %We optimize both within view relationship and between views relationship among kernel values. 
The novelty of the proposed approach is in modelling the between-view relationships as follows: (1) To complete kernel matrices, we restrict the individual normalized kernel matrices corresponding to each view in the convex hull of normalized kernel matrices of other views. (2) To propagate relevant information across views, we propose a novel approach of restricting  the local embedding of one view in the convex hull of local embeddings of other views. While local embeddings are found by representing  each feature representation for a kernel as a sparse linear combination of other available feature representations which is also called as  basis vectors. We assume that basis vectors of each view is in the convex hull of basis vectors of other views.


The concept of restricting a kernel matrix in the convex hull of other kernel matrices has been already used in the field of multiple kernel learning \citep{lan04,bac04,arg05} and kernel alignment \citep{cri06,cor12} when all kernel matrices are complete. But in this paper we explore this idea to complete kernel matrices of individual views with the help of all incomplete kernel matrices of other views by simultaneously completing all of them. Again, the concept of local linear embeddings has been also used for multi -view clustering \citep{she13} where all views are assumed to have exactly same embedding. While our method is able to  model not only same but also similar embeddings of different views. 
%Hence the model can also capture heterogeneous relationship among views.

It is important to note that, the proposed model automatically decides the number of basis vectors of each view while simultaneously representing all data points with help of them and restricting these basis vectors in the convex hull of basis vectors of other views. The non-linearity of individual kernel functions are also preserved in the basis vectors which define the corresponding embeddings.

%the dimension of local embeddings varies across views depending on non-linearity of the corresponding kernel function. Also the effective dimension of embeddings of individual views is defined by the number of selected basis vectors.  The proposed model automatically decides the number of basis vectors of each view while simultaneously representing all data points with help of them and restricting these basis vectors in the convex hull of basis vectors of other views. The non-linearity of individual kernel functions is also preserved in the kernel among basis vectors which define the corresponding subspace.

As the proposed model need to solve a non-convex optimization problem which we solve efficiently by block-wise  proximal gradient descend.
%simultaneously learn  the view specific subspaces, embeddings of all data points on it by restricting it to be on convex hull of other related views,  solving this problem efficiently is a daunting task. We solve the 





%The proposed method restrict the completed kernel matrix for  individual view in a positive semi-definite cone. For computation efficiency and also to put additional regularization on completed kernel matrix  we propose a sparse approximation of kernels by finding a view specific local linear embedding for all data points in each view. We re-present  each features maps for a kernel as linear combination of a sparse subset of other feature maps corresponding to available rows or columns of it.  We name them as the basis vectors. The linear weights are called as basis weights. This concept is similar to Nystr{\" o}m methods \citet{ dri05} but the main difference between the proposed method and the Nystr{\" o}m method lies in the selection of columns or basis. We select those which are most effective for best kernel approximation for a group of homogeneous views while Nystr{\" o}m method follow random selection. Moreover,  Nystr{\" o}m method selects a single subset of columns to express all other data points while the proposed method are allowed to select different set of basis vectors for a different set of data points.  

%To propagate relevant information across views,  It exploit the concept of restricting completed kernel matrix of one view on convex hull of kernels of other related views following the multiple kernel learning method \citet{lan04,bac04}.We restrict the individual normalized kernel matrix corresponding to each view on a convex hull of normalized kernel matrices of other views by following \citet{arg06Finally we extend this idea by restricting basis weights of one view on convex hull of basis weights of other views and learn completed kernel by learning underlying embedding of all views collectively. 

 

 
 
%Restricting the  kernel of each view on the  convex hull of kernels of other views  restrict the kernel values  to have same underlying distribution for all views. It is useful to exploit across-view similarity among their underlying embeddings.  When modelling multi-view embedding \citet{she13} has assumed to have same local linear embedding in all views. But this restrict all embeddings are to be exactly same. To make our model enough flexible to capture the relationship of not only exactly same embeddings but also similar embeddings, we propose a novel approach of restricting  the embedding of one view on the convex hull of embeddings of other similar views.



%Once we know the embeddings of data-points in an individual subspace of a view and the relationship among embeddings across the  homogeneous views,  we can extrapolate the position of one data-point in one view to another subspace of another view where its feature-map is missing. In this way we are able to embed all missing feature-maps in all views simultaneously even if  any complete kernel matrix is not available. 


%As a result, the proposed model is not only able to model the highly non-linear kernels for individual views, it is also able to model non-linear relationships among kernels of different views.  Moreover, simultaneous prediction approach enable us to capture the required information from other views with missing values and it has no need of any complete view.  More importantly the predicted complete kernel gram matrix will also satisfy positive semi definite property without any explicit low rank assumption.



%We have defined a non-convex optimization problem but without  any positive semidefinite cone constraint which has been efficiently solved by  solving a sequence of convex problem.



==> pexp.tex <==
 \section{PLAN FOR EXPERIMENT SECTION}

\paragraph{TOY}
\begin{itemize}
\item To study performance of all method with respect to eigen spectrum : DONE

\begin{itemize}
\item Observation :
\item If underlying subspaces and kernel values does not match then  Equation(\ref{eqn:impute}) perform best
\item  When views are highly non-linear   then PSD formulation is better than approximation
\end{itemize}
\item To study Stability of $\bA$ : need to plan
\end{itemize}

\paragraph{DREAM and RCV}
\begin{itemize}
\item  Real world  application
\item RCV : this dataset is more useful for showing retrieval task. 
\end{itemize}

\paragraph{STUDY}
\begin{itemize}
\item REPORT prediction error (RMSE , Correlation (to show retrieval task) )
\begin{itemize}
		\item average 
                   \item view-wise (for analysis)
                   \item how it varies with non-linearity of kernel
		\item how it varies with increase of missing views 
\end{itemize}
\item Contribution over EM :  even when one view present but eigen spectrum of two views are not same then  proposed method perform better that em based method
\item COMPARE with NYSTROM heuristic :  comparative but very fast compare to FINAL method
\end{itemize}


==> relate.tex <==
\section{Related Work}

In this section I will mention Graepel single view kernel completion and describe EM based method and also generative model based method to model similarity matrices.
